Learning from Synthetic Animals

Despite great success in human parsing, progress for parsing other deformable articulated objects, like animals, is still limited by the lack of labeled data. In this paper, we use synthetic images and ground truth generated from CAD animal models to address this challenge. To bridge the domain gap between real and synthetic images, we propose a novel consistency-constrained semi-supervised learning method (CC-SSL). Our method leverages both spatial and temporal consistencies, to bootstrap weak models trained on synthetic data with unlabeled real images. We demonstrate the effectiveness of our method on highly deformable animals, such as horses and tigers. Without using any real image label, our method allows for accurate keypoint prediction on real images. Moreover, we quantitatively show that models using synthetic data achieve better generalization performance than models trained on real images across different domains in the Visual Domain Adaptation Challenge dataset. Our synthetic dataset contains 10+ animals with diverse poses and rich ground truth, which enables us to use the multi-task learning strategy to further boost models' performance.

==> exp_results.tex <==
\section{Experiments}
    Where to put real models work worse for cows, pony but synthetic model works well?

    1. How we split the TigDog dataset by video.
    
    2. Stacked Hourglass training parameters.

\subsection{Keypoints detection on TigDog}
    In this section, we show different models' performances on TigDog val dataset.

    \begin{table*}[h]
    \centering
    \begin{tabular}{cccc|cccccccc} 
    \hline       \hline
    \multicolumn{4}{c}{Models} & \multicolumn{8}{c}{Accuracy}
    \\ 
    Data  & Strong Aug & SSL &  & Eyes & Chin & Shoulders & Hip & Elbows & Knees & Hooves & Mean\\ [0.5ex] \hline 
    Real  & & & & 85.38 & 88.01 & 64.33 & 93.73 & 83.58 & 80.53 & 72.11 & 78.91\\
    Real  & \checkmark & & & 81.31 & 87.12 & 70.22 & 86.13 & 82.41 & 81.32 & 72.14 & 78.44\\
    Synthetic &  & & & 45.70 & 57.15 & 25.03 & 25.90 & 21.30 & 24.28 & 17.23 & 25.46\\
    Synthetic & \checkmark & & & 66.58 & 82.63 & 56.46 & 66.65 & 55.12 & 57.61 & 48.91 & 59.44\\
    % Synthetic & & \checkmark & & 0 & & & & & & & 0\\
    Synthetic & \checkmark & \checkmark & & 79.42 & 91.65 & 46.71 & 85.67 & 70.15 & 69.01 & 60.30 & 71.26\\
    % Synthetic & \checkmark & \checkmark & \checkmark & 0 & & & & & & & 0\\
    \hline

    \end{tabular}
    \caption{Horse Keypoints Prediction PCK@0.05. Synthetic data are with random background and random textures.}

    \end{table*}

    \begin{table*}[h]
    \centering
    \begin{tabular}{cccc|cccccccc} 
    \hline       \hline
    \multicolumn{4}{c}{Models} & \multicolumn{8}{c}{Accuracy}
    \\ 
    Data  & SA & SSL & MT & Eyes & Chin & Shoulders & Hip & Elbows & Knees & Hooves & Mean\\ [0.5ex] \hline 
    Real  & & & & 96.74 & 95.54 & 62.14 & 91.47 & 71.16 & 78.85 & 81.39 & 82.07\\
    Real  & \checkmark & & & 91.11 & 87.49 & 62.09 & 78.78 & 68.07 & 74.31 & 77.86 & 76.80\\
    Syn & & & & 15.58 & 16.56 & 11.02 & 52.06 & 15.07 & 13.61 & 15.25 & 16.98\\
    Syn & \checkmark & & & 23.80 & 44.41 & 21.87 & 61.78 & 31.49 & 29.36 & 37.80 & 40.48\\
    % Syn & & \checkmark & & 0 & & & & & & & 0\\
    Syn & \checkmark & \checkmark & & 37.37 & 55.63 & 16.31 & 73.67 & 48.67 & 27.91 & 52.37 & 54.52\\
    Syn & \checkmark & \checkmark & \checkmark & 0 & & & & & & & 0\\
    Syn+Real & & & & 0 & & & & & & & 0\\
    \hline

    \end{tabular}
    \caption{Tiger Keypoints Prediction PCK@0.05. Synthetic denotes models trained with random background and random texture.}

    \end{table*}

\subsection{Model Generalization}
    In this section, we test models' generalization power on images from Visual Domain Adaptation Challenge dataset (VisDA2019). The dataset contains six domains. We manually annotate images from each domain.




\subsection{Ablation Experiments}

    \subsubsection{CycleGAN and Adversarial Training}


    \subsubsection{Part Segmentation}

    \subsubsection{Tiger combined dataset}
    
    \subsubsection{Other Animals}
    

    \subsubsection{Dense Keypoints}
    1. Number of synthetic images.
    
    2. $\lambda$ study
    real/synthetic balance: Varying $\lambda$ from 0 to 1. 
    
    3. Explain why CycleGAN(visually) and gradient reversal fails?
    
    3.1. CycleGAN generate unrealistic images.
    
    3.2. Feature level adversarial training can learn a separate model for both datasets as feature dimensions are too high. Therefore, it doesn't make sense to enforce features to merge between datasets.

\subsection{Other animals}
    Qualitatively show performances on tigers, cats or cows
    
    
    \begin{table*}[h]
    \centering
    \begin{tabular}{cccc|cccc|cccc} 
    \hline       \hline
    \multicolumn{4}{c}{Models} & \multicolumn{4}{c}{Visible Kpts Accuracy} & \multicolumn{4}{c}{Full Kpts Accuracy}
    \\ 
    Data  & SA & SSL & MT & Sketches & Paintings & Cliparts &  & Sketches & Paintings & Cliparts & \\ [0.5ex] \hline 
    Real  & & & & 79.03 & 79.49 & & & 81.67 & 77.78 & \\
    Real  & \checkmark & & &  &  & & &  &  &\\
    % Synthetic & & & & 0 & 0 & & 0 & 0 & &\\
    Synthetic & \checkmark & & &  & & & & &  &\\
    % Synthetic & & \checkmark & & 0 & & & 0 & 0 & &\\
    Synthetic & \checkmark & \checkmark & & 79.87 & 78.88 & & & 81.67 & 80.56 &\\
    Synthetic & \checkmark & \checkmark & \checkmark & 0 &  & & & 0 & &\\
    \hline

    \end{tabular}
    \caption{Horse Keypoints Prediction on VisDA2019 PCK@0.1}

    \end{table*}

    \begin{table*}[h]
    \centering
    \begin{tabular}{cccc|cccc|cccc} 
    \hline       \hline
    \multicolumn{4}{c}{Models} & \multicolumn{4}{c}{Visible Kpts Accuracy} & \multicolumn{4}{c}{Full Kpts Accuracy}
    \\ 
    Data  & SA & SSL & MT & Sketches & Paintings & Cliparts & & Sketches & Paintings & Cliparts & \\ [0.5ex] \hline 
    Real  & & & & 68.09 & 81.02 & 86.60 & & 61.67 & 73.33 & 80.86 \\
    Real  & \checkmark & & & 61.51 & 69.40 & 83.30 & & 58.89 & 65.50 & 79.81\\
    % Synthetic & & & & 0 & 0 & & 0 & 0 & &\\
    Synthetic & \checkmark & & & & & & & & &\\
    % Synthetic & & \checkmark & & 0 & & & 0 & 0 & &\\
    Synthetic & \checkmark & \checkmark & & 82.48 & 70.43 & 77.44 & & 78.33 & 68.33 & 75.31 \\
    Synthetic & \checkmark & \checkmark & \checkmark & 0 &  & & & 0 & &\\
    \hline

    \end{tabular}
    \caption{Tiger Keypoints Prediction on VisDA2019 PCK@0.1}

    \end{table*}
